Microfabrication techniques for trapped ion quantum information processing

Quantum-mechanical principles can be used to process information (QIP). In one approach, linear arrays of trapped, laser cooled ion qubits (two-level quantum systems) are confined in segmented multi-zone electrode structures. The ion trap approach to QIP requires trapping and control of numerous ions in electrode structures with many trapping zones. I investigated microfabrication of structures to trap, transport and couple large numbers of ions. Using 24Mg+ I demonstrated loading and transport between zones in microtraps made of boron doped silicon. This thesis describes the fundamentals of ion trapping, the characteristics of silicon-based traps amenable to QIP work and apparatus to trap ions and characterize traps. Microfabrication instructions appropriate for nonexperts are included. Ion motional heating was measured. <<>> Using MEMs techniques I built a Si micro-mechanical oscillator and demonstrated a method to reduce the kinetic energy of its lowest order mechanical mode via capacitive coupling to a driven radio frequency (RF) oscillator. Cooling resulted from a RF capacitive force, phase shifted relative to the cantilever motion. The technique was demonstrated by cooling the 7 kHz fundamental mode from room temperature to 45 K. <<>> I also discuss an implementation of the semiclassical quantum Fourier transform (QFT) using three beryllium ion qubits. The QFT is a crucial step in a number of quantum algorithms including Shor's algorithm, a quantum approach to integer factorization which is exponentially faster than the fastest known classical factoring algorithm. This demonstration incorporated the key elements of a scalable ion-trap architecture for QIP.

==> apparatus/figures/transfig.tex <==
\typeout{TransFig: figures in epic.}
\usepackage{epic}

\endinput


==> introduction.tex <==
\clearpage
\chapter{Introduction}

Quantum-mechanical principles can be used to process information. In one
approach, linear arrays of trapped, laser cooled ion qubits (two-level quantum
systems) are confined in segmented multi-zone electrode structures
\cite{cirac1995a,bible,kielpinski2002a,monroe2008a,blatt2008a}. Strong Coulomb
coupling between ions is the basis for quantum gates mediated by phonon exchange.
Applications of Quantum Information Processing (QIP) include solution of
problems believed to be intractable on classical computers.  The ion trap
approach to QIP requires trapping and control of numerous ions in electrode
structures with many trapping zones.  In addition to QIP, ion traps are versatile tools found in applications
including mass spectroscopy ~\cite{paul1990a}, precision atomic
\cite{schmidt2005a} and molecular spectroscopy \cite{vogelius2004a,schmidt2006b},
and tests of fundamental physics \cite{van-dyck-jr1987a,russell-stutz2004a}.

In this thesis I discuss microfabrication and testing of miniature linear RF Paul
traps intended for use in ion QIP experiments. The aim of this effort was
demonstration of traps with ion-electrode separation below $50~\mu \text{m}$ and
investigation of microfabrication technologies amenable to building of large
trap arrays.   At the outset of my work the state of the art was three-dimensional
gold-coated alumina structures resembling 4-rod RF quadrupole traps.  In
practice, this technology could not be scaled to trap and manipulate large
numbers of ions. Moreover, fabrication and testing of trap structures was time-consuming and
expensive. To address these shortcomings I investigated microfabricated
structures to trap, transport and couple many ions.

Among several candidate fabrication techniques, I focused on making trap
electrodes out of boron doped silicon.  With sufficient doping, silicon is an
adequate electrical conductor and can be precisely micromachined.  Boron doped
silicon ion traps have several advantages: tools for processing silicon are
ubiquitous in microfabrication facilities; the process uses only silicon, so it
is compatible with CMOS foundry processes; surfaces exposed to trapped ions have
low surface roughness ($<$~1~nm~RMS); high aspect ratio structures $100$'s~$\mu
\text{m}$ tall are possible; and stray fields from exposed dielectric surfaces
are negligible. The doped silicon traps I demonstrated traps included two-layer
and surface electrode geometries. The latter geometry is especially amenable to a
variety of microfabrication techniques since all trap features lie in a single
plane. In my traps single $^{24}$Mg$^+$ ions were trapped as near as
$40~\mu\text{m}$ to the electrodes.  All fabrication work was done in-house at the NIST
microfabrication facility.  It is straightforward to build boron doped traps with
electrodes as small as $5~\mu\text{m}$.

A key performance characteristic of ion traps is the rate at which ion motional
modes heat. In my traps upper bounds on heating were determined; however, heating due to
externally injected noise could not be completely ruled out.  Noise on the RF
potential responsible for providing confinement was identified as one source of
injected noise.  Limits on heating from a variety of sources were calculated and
the results of several related experiments are presented.

As a result of my work the time required to design, fabricate, and load ions into
a new trap structure was reduced from around one year to less than a month.
Besides microfabrication, several new techniques were developed to accelerate
trap testing.  These included streamlined layout and simulation software, a new
rapid turn-around vacuum apparatus, plug and play chip carrier technology, the
use of $^{24}$Mg$^+$ (which has a simplified atomic structure relative to
$^{9}$Be$^+$, our usual ion qubit) and dedicated laser systems for Doppler
cooling and photoionization.

The first Section of this thesis describes the fundamentals of ion trapping, the
characteristics of silicon-based traps amenable to QIP work and apparatus to trap
ions and characterize traps.  In the introductory chapter, the dynamics of ions
confined in Paul traps based on the pseudopotential approximation is presented.
Subsequent topics include numeric and analytic models for various Paul trap
geometries, a list of considerations for practical trap design and an overview of
microfabricated trapping structures. The Apparatus chapter discusses in detail
the techniques needed to trap and Doppler laser cool $^{24}$Mg$^+$ ions.
It also provides details including specific part numbers for the vacuum apparatus. A
lengthy Appendix on microfabrication was written with atomic physicists in mind;
it includes step by step instructions appropriate for nonexperts.  Throughout,
the level of detail is intended to be sufficient so that a physicist with
background in atomic physics and access to a fabrication facility should be able
to reproduce the traps and experiments I conducted.
 
Using the microfabrication technology developed for ion traps, I also made a
cantilevered micromechanical oscillator and with coworkers demonstrated a method
to reduce the kinetic energy of its lowest order mechanical mode via its capacitive coupling to
a driven RF resonant circuit. Cooling results from a RF capacitive force, which
is phase shifted relative to the cantilever motion. The technique was
demonstrated by cooling a 7~kHz mode from room temperature to $45$~K. Ground
state cooling of the mechanical modes of motion of harmonically trapped ions is
routine; equivalent cooling of a macroscopic harmonic oscillator has not yet been
demonstrated. Extension of this method to devices with higher motional
frequencies in a cryogenic system, could enable ground state cooling and may
prove simpler than related optical experiments.

I also discuss an implementation of the semiclassical quantum Fourier transform
(QFT) using three beryllium ion qubits.  The QFT is one of several QIP algorithms
demonstrated in NIST gold-on-alumina ion traps. The QFT is a crucial step in a
number of quantum algorithms including Shor's algorithm, a quantum approach to
integer factorization which is exponentially faster than the fastest known
classical factoring algorithm. This demonstration incorporated the key elements
of a scalable ion-trap architecture for QIP.

==> rfam/rfam.tex <==

 

 








